Spherical clustering of users navigating 360{\deg} content

In Virtual Reality (VR) applications, understanding how users explore the omnidirectional content is important to optimize content creation, to develop user-centric services, or even to detect disorders in medical applications. Clustering users based on their common navigation patterns is a first direction to understand users behaviour. However, classical clustering techniques fail in identifying these common paths, since they are usually focused on minimizing a simple distance metric. In this paper, we argue that minimizing the distance metric does not necessarily guarantee to identify users that experience similar navigation path in the VR domain. Therefore, we propose a graph-based method to identify clusters of users who are attending the same portion of the spherical content over time. The proposed solution takes into account the spherical geometry of the content and aims at clustering users based on the actual overlap of displayed content among users. Our method is tested on real VR user navigation patterns. Results show that our solution leads to clusters in which at least 85% of the content displayed by one user is shared among the other users belonging to the same cluster.

==> ICASSP_2019/GeoDistance_2.tex <==

	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\section{Geodesic distance as proxy of viewport overlap } %metric}	
	\label{sec2}
	%\textbf{Why Geodesic Distance as proxy?}\\
%Our goal is to identify clusters of users who are displaying the same portion of spherical content within a frame or over a series of consecutive frames. We derive a similarity metric that reliably quantifies how similar the portions attended by two users are. %users are  similar in terms of their displayed   portion of the spherical content. 
A key aspect of our clustering algorithm is to group users based on a metric that reliably reflects users similarities during the navigation. We argue that similarity in the navigation is captured by viewport overlap. In this section, we identify a metric that reliably reflects this overlap.
More specifically, each user attends a portion of the spherical surface. This is the projection on the spherical surface  of a plane tangent to the sphere (\ie \textit{viewport}) in the point that identifies the user's viewing direction (\textit{center of the viewport})%(Figure~\ref{viewport})
\footnote{Without loss of generalization, we consider a scenario in which the viewports of all users have the same horizontal and vertical field of view.}.
% we   refer to the \textit{viewport} as the portion of the spherical surface attended by the user and to the \textit{center of the viewport} as the viewing direction. 
%Our goal is to identify similar users, with the similarity expressing how closely users are looking at the same portion of the spherical content. This translates into an overlap metric, expressing the pairwise overlap subsisting between viewports displayed by two users in the same time frame. 
%	A key aspect to group users with common viewports   is to find a meaningful similarity metric that extract this information without adding computational complexity. 
The overlap between the viewports attended by two users at an instant in time is a clear indicator of how  similar users are with respect to their displayed  viewports.  For example,  an overlap equal to the area of the viewport corresponds to two users attending exactly the same portion of visual content. The geometric overlap could be analytically computed, knowing the rotation associated to each user head's position (\ie roll, pitch, and yaw) and the horizontal and vertical fields of view that define the viewport. However, this is non trivial since it requires to evaluate closed-form expression of the viewport on the sphere. % and time-consuming computation with a large number of users.
Here, we show that the \textit{geodesic distance} between two viewport centres under specific settings acts as proxy of the viewport overlap. Thus, we propose the simple and straightforward solution of using this distance  as a proxy for viewport overlap. 

The geodesic distance is the length of the shortest arc connecting the viewport centers on the sphere.
%In order to define 
%Since viewports whose centers are at the same geodesic distance could have different viewport overlap.
Such distance is an approximation of the actual area overlap as it does not account for the three degrees of freedom of the user's head rotation, which defines the exact viewport. As a result, viewports whose centers have the same geodesic distance could correspond to a different viewport overlap due to the intrinsic approximation error (example in Fig.~\ref{fig_ch04:VPs_intersec}).
%. The geodesic distance between the two viewport's centres is  ${\pi}/{8}$ in both cases Figure~\ref{fig_ch04:VPs_intersec}(a) and (b). However, the green viewport in the second figure is rotated of $ {\pi}/{2}$. Even if it is an extreme situation, this rotation reduces the overlap from 87\%  to 58\% of the total area. It follows that the the geodesic distance is an approximation (and not exact reflection) of the viewport overlap.
Nevertheless, the smaller the distance between viewport centers, the smaller the approximation error with geodesic distance. As an example, Fig.~\ref{fig:ComparisonUser1} shows the pairwise geodesic distance (in blue) and the pairwise area overlap (in red) between the viewport attended by one user and those of 58 other users, for a frame of a video sequence, extracted from the public dataset proposed in \cite{corbillon2017}. %in Rollercoster frame presented in Figure~\ref{fig:1_selected_frames} (a). %In particular, 
The correlation between the two metrics is evident: if the overlap is high, the geodesic distance between the two viewport centres is low. Particularly, a viewport area overlap that is larger than 75\% of the viewport area corresponds to a geodesic distance smaller than ${3\pi}/{4}$.  We are therefore interested in identifying a threshold value below which the geodesic distance is a robust proxy of the viewports overlap.  \\
To empirically define this  threshold, we built the \ac{ROC}  curve as follows.   We assume that two users are attending   the same portion of   content if their viewports overlap by at least $O_{{th}}$ of the total viewport area. We then define a threshold value for the geodesic distance $G_{th}$ such that  users are attending the same content if their geodesic distance is below threshold. Anytime users are separeted by a geodesic distance lower than $G_{th}$ and the overlap of their viewport is less than $O_{{th}}$, we experience a false positive. Conversely, a true positive is experienced if users separated by a geodesic distance above the threshold but experience a viewport overlap equal or higher than $O_{{th}}$. Equipped with these definitions, we can compute the ROC  by considering all the videos and user' navigation patterns included in the dataset described in \cite{corbillon2017}.
%We assume that two users are attending at the same portion of visual content if their viewports overlap by at least 80\% of the total viewport area.
%The event to detect is a viewport overlap over 80\% of the total viewport area by pairwise geodesic distance. The threshold to test is the geodesic distance, $G_{th}$. 
Fig.~\ref{fig:ROC} shows the curve obtained in our scenario with $O_{th}=80\%$.
%Figure~\ref{fig:ROC} also shows the \ac{ROC} curve obtained by considering all the videos included in the dataset described in \cite{corbillon2017}. 
On the x axis of the ROC curve there is the \ac{FPR}, \ie the probability to have a wrong classification over the number of actual negative events. This rate should be as small as possible. On the contrary, the \ac{TPR} on the y axis represents the probability to correctly classify an event.
The best value of geodesic distance is ${\pi}/{10}$ since it corresponds to a \ac{TPR} value equal to 1, which in our application means a sure identification of viewports with an overlap of at least 80\% based on the geodesic distance between their centers. %For our application, we want to be sure to detect all the couples of viewports that do have a significant overlap. %, and we can tolerate to have an optimistic prediction.
Therefore, in the following  we assume $G_{th} = {\pi}/{10}$ as a suitable threshold to reliably approximate the area overlap between two viewports by means of the geodesic distance between their centers.
%\noteSR{In teh following, we have define geodesic threshould as $G_th$.}
%\begin{figure}[t]
%	\centering
%		\includegraphics[width=0.5\textwidth]{figures/ROC_Diving_Roller.eps}
%	\caption{\label{fig:ROC} \noteSR{Do we want to put also the ROC figure for these two videos?}.}
%\end{figure}
%	We propose to use the pairwise geodesic distance between viewport's centres as proxy of the corresponding overlap between the two user's viewports.

% Therefore, in this paper we aims at finding a threshold value % optimal threshold value
 	%However, evaluating the viewport overlap   is non trivial and time-consuming, especially in a scenarios with a large number of users.
	%Therefore, there is the need to introduce a simpler metric  that can act as a proxy for the viewport overlap. The straightforward intuition is to evaluate the distance between viewports centers and use this  as metric distance that reflects the viewports overlap. To take into account for the spherical geometry, we consider the  \textit{geodesic distance}, which measures the shortest route between two points on a sphere.  However, it is worth mentioning that users at the same geodesic distance could have different viewport overlap. Namely, the geodesic distance  does not account for the full head-movements of user. In particular, the rotation of the viewport on the plane x-y is neglected as shown in the example of Figure~\ref{fig_ch04:VPs_intersec}. The geodesic distance between the two viewport's centres is  ${\pi}/{8}$ in both cases Figure~\ref{fig_ch04:VPs_intersec}(a) and (b). However, the green viewport in the second figure is rotated of $ {\pi}/{2}$. Even if it is an extreme situation, this rotation reduces the overlap from 87\%  to 58\% of the total area. It follows that the the geodesic distance is an approximation (and not exact reflection) of the viewport overlap. The closest the viewports centers (i.e., the smaller the distance) the smaller is the approximation error in taking into account the geodesic distance rather than the viewport overlap. At the same time, for large distances, the approximation error can be substantial. Therefore, in this paper we aims at finding a threshold value % optimal threshold value
 %$G_{th}$% has to be define 
 % that minimize the discrepancy between these two metrics. %\noteLT{even if we don't have the ROC curve, I would still say that you evaluate it via ROC. Otherwise it is not clear how you do it and I believe that this is a contribution (the fact that you don't simply use the metric but you impose a threshold value is a contribution).}
	\begin{figure}[t]
		\centering
		\subfigure[$87\%$ overlap]{
			\includegraphics[width=0.15\textwidth]{figures/VPinter_1.eps}}
			\hfil		%IIntersecVPs_1.eps}}
		\subfigure[$58\%$ overlap ]{
			\includegraphics[width=0.15 \textwidth]{figures/VPinter_2.eps}}		%IntersecVPs_2.eps}}\\
		\caption{\label{fig_ch04:VPs_intersec} Viewports (in green and blue) with ${\pi}/{10}$ centre distance.  (a) viewports are aligned with an overlap of $87\%$, (b) one viewport is rotated by ${\pi}/{2}$ resulting an overlap of  $58\%$.}
	\end{figure}
	 \begin{figure} 
	\centering
	%\subfigure[Comparison pairwise geodesic distance and viewport overlap in Rollercoaster]{
		\includegraphics[width=0.40\textwidth]{figures/GeodvsOver_Roller.eps}
%	\subfigure[Timelapse]{
%		\includegraphics[width=0.40\textwidth]{figures/ROC.eps}}
	\caption{Comparison between pairwise geodesic distance and viewport overlap in one frame of video Rollercoaster from \cite{corbillon2017}. } %The geodesic distance is plotted with inverse y axis making correspond low value of geodesic distance to high value of overlap.}
	 \label{fig:ComparisonUser1}
\end{figure}
%
	% and is easy to evaluate.
	%(by calculating Equation~\ref{eq: GeodDistance}) and at the same time it takes into account the spherical geometry of the content.. 
	%\noteSR{should I put math equation?}
%	In particular, given two points, $A$ and $B$, with longitude, $\theta_A$ and $\theta_B$, and latitude, $\phi_A$ and $\phi_B$ respectively, the geodesic distance can be evaluated as follow: 
%	\begin{equation}
%	\begin{split}
%	GeodDist(A,B) = &\arccos( \sin(\phi_A)\sin(\phi_B) + \\ 
%	&\cos(\phi_A) \cos(\phi_B)\cos(\theta_B - \theta_A) ).
%	\end{split}
%	\label{eq: GeodDistance}
%	\end{equation} 
	%\textbf{Relation btw geodesic distance and VP overlap}\\
	%In the example actually, the value of overlap are  proving the geodesic distance is still meaningful as approximation of an optimal threshold value $G_{th}$ has to be define to minimize the discrepancy between these two metrics.\\
%
%	To further demonstrate the validity of our assumption, we consider %a real \ac{VR} scenario, using 
%	the  public dataset presented in \cite{corbillon2017} composed by five videos, one minute long and watched by 59 users. 
%	%Due to limited space, in the following we present the analysis to define the optimal threshold $G_{th}$ only for two videos of the dataset: 
%	As example, Figure~\ref{fig:1_selected_frames} shows the position of viewport’s centres in two selected frames of two videos of the dataset,  Rollercoaster and Timelapse.\footnote{For the sake of clarity, these viewports’ positions are represented by their centre on the projected panorama rather than on the original spherical domain.} Rollercoaster has one main \ac{FoA} (i.e., the rail) while in Timelapse, there are many fast moving objects (e.g., buildings, people) along the equator line.  %We chose these videos in order to have a simple but complete scenario.  %The users' behaviour perfectly matches with the above mentioned content features.
%% \red{In Rollercoaster,  Figure~\ref{fig:1_selected_frames} (a), most of the people are focused on the same area (one \ac{FoA}) and only few of them are looking in other directions. On the contrary, the position of users in Timelapse is more scattered as shown in Figure~\ref{fig:1_selected_frames} (c). However, it is still possible to identify small groups with similarities in terms of positions (for instance, most of the people are displaying the central building). }\noteLT{I would remove this part and here be focus on the geodesic distance.}
%	\begin{figure}[t]
%	\centering
%	%	\subfigure[Users position at Rollercoaster frame = 1480]{
%	%\includegraphics[width=0.23\textwidth]{figures/Fig3_Roller__1480.eps}}
%	\subfigure[Rollercoaster frame = 1480]{
%		\includegraphics[width=0.23\textwidth]{figures/Roller_frame1480.eps}}
%	%	\subfigure[Users position at Timelapse  frame = 1228]{
%	%		\includegraphics[width=0.23\textwidth]{figures/Fig3_Time_1228.eps}}
%	\subfigure[Timelapse frame = 1228]{
%		\includegraphics[width=0.23\textwidth]{figures/Times_frame1228.eps}}
%	\caption{\label{fig:1_selected_frames} Example of analysed video content with user viewport's centres in green.}
%\end{figure} 
%To better understand correlation between geodesic distance and viewport overlap, %we select one user (i.e., User 1) as reference and evaluate both pairwise metrics for each other users. Results are provided in 
%Figure~\ref{fig:ComparisonUser1} (a) show the pairwise geodesic distance (y axis in blue) and the pairwise overlap (y axis in red) between one user as reference (i.e., User 1) and others in Rollercoster frame presented in Figure~\ref{fig:1_selected_frames} (a). %In particular, 
%%hows results for the selected frames provided in Figure~\ref{fig:1_selected_frames}. %these two metrics 
%The geodesic distance has been plotted with inverse y axis in order to make correspond low value of geodesic distance to high value of overlap.
%The correlation between the two metrics is evident: if the overlap is high, the geodesic distance between the two viewport centres is low. %\noteLT{When you describe the figure I would say that the distance is plotted in the reverse order in such a way that small distances are on the top.}%Moreover, the red points in the plots correspond to users with pairwise overlap over than the $80\%$.
%Particularly, a viewport area overlap larger than 75\% of the viewport area corresponds to a geodesic distance smaller than ${3\pi}/{4}$. %looking at the corresponding value of geodesic distance, we can notice that most of the users are at a reduced distance from the reference user, in most of the case this distance is ${\pi}/{10}$.  
%\begin{figure}[t]
%	\centering
%	\subfigure[Comparison pairwise geodesic distance and viewport overlap in Rollercoaster]{
%		\includegraphics[width=0.40\textwidth]{figures/GeodvsOver_Roller.eps}}
%	\subfigure[Timelapse]{
%		\includegraphics[width=0.40\textwidth]{figures/ROC.eps}}
%	\caption{\label{fig:ComparisonUser1} .} %The geodesic distance is plotted with inverse y axis making correspond low value of geodesic distance to high value of overlap.}
%\end{figure}
%Looking at the corresponding value of geodesic distance, we can notice that most of the users are at a reduced distance from the reference user, in most of the case this distance is ${\pi}/{10}$.  
%
%[\textbf{ROC analysis to formalize geodesic threshold?}]\\
%To formalise the threshold $G_{th}$, we further extend the analysis to all video in the dataset \cite{corbillon2017}. As typical in a classification problem, we used a \ac{ROC} curve. This graph shows clearly the performance for a classification algorithm for different values of thresholds. On the x axis, there is the \ac{FPR}, probability to have a wrong classification over the number of actual negative events. This rate should be as small as possible. On the contrary, \ac{TPR}, is on the y axis and it is the probability to correctly classify an event. In our case, the event to detect is a viewport overlap over 80\% of the total area by pairwise geodesic distance. While the threshold to test is the geodesic distance. The best value of geodesic distance is $\frac{pi}{10}$ since it corresponds to a \ac{TPR} value equal to 1, which in our application means a strong matching of neighbours detected with the overlap and the geodesic distance. For our application, we want to be sure to detect all the couple of neighbour and we can tolerate to have an optimistic prediction. Therefore in the following, we assume $G_{th} = {\pi}/{10}$ as a suitable threshold to approximate the geodesic distance as a consistent overlap between two viewports.




==> ICASSP_2019/algo.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Clique-Based Clustering Algorithm}

We now describe the proposed clustering algorithm, aimed at identifying clusters of users having a common viewport overlap.
%only among users that have at most a distance of $G_{th}$, which is the threshold distance ensuring a minimum viewport overlap as proved in the previous section.   
%Users displaying frame $t$ are represented by the graph 
%A graph is a data structure composed by a finite set of \emph{vertices} or \emph{nodes} that might be connected each other by \emph{edges} based on their similarities \cite{tan2013data}. In graph theory, clustering or community detection algorithms identify groups of nodes that are more densely connected to each others than to others. An ideal cluster manages to minimize the intra-cluster distance (i.e., the distance between elements belonging to the same cluster) and maximize the inter-cluster distance (i.e., the distance between elements belonging to the different cluster).\\
We model the evolution of users' viewports over a time-window $T$ as a set of graphs $\{ \mathcal{G}_t\}_{t=1}^T$. Each unweighted and undirected  graph $\mathcal{G}_t = \{\mathcal{V}, \mathcal{E}_t, \text{W}_t \}$ represents  the set of users\footnote{Without loss of generality, we assume that the set of users does not change over time. This covers also cases in which users' devices are not synchronized in the acquisition time, as users' positions are usually interpolated to create a synchronized dataset. } navigating over time, where $\mathcal{V}$ and $\mathcal{E}_t$ denote the node and edge sets of $\mathcal{G}_t$. Each node in  $\mathcal{V}$ corresponds to a user interacting with the 360$^\circ$ content at instant $t$. Each edge in $\mathcal{E}_t$ connects neighbouring nodes, where two nodes are neighbours if the geodesic distance between the viewport centers associated to the users represented by the nodes is lower than $G_{th}$ , as defined in Section II. The binary matrix $\text{W}_t$ is the adjacency matrix of $\mathcal{G}_t$, with $w_t(i,j)=1$ if users are neighbors. More formally:
%We represent users on the sphere at a particular instant $t$ by the graph $\mathcal{G}_t = \{\mathcal{V}, \mathcal{E}_t, \text{W}_t \}$,  where each node  $v\in\mathcal{V}$ identifies one user. Two users $i$ and $j$ are defined as \textit{adjacent} or \textit{neighbours} and then they are connected each other by an \emph{edge} $\mathcal{E}$ based on their similarities. The geodesic distance is used as similarity metric to decide if nodes are connected among each other. W is the adjacency matrix that define neighbours in the graph. When $\{i,j\} \in \mathcal{E}$, the entry $W(i,j)$ is defined as following:
\begin{equation}
	w_t(i,j) = 	 \begin{cases} 
	1,    & \mbox{if } g(i,j) \leq G_{th} \\ 
	0, & \text{otherwise} \\
	\end{cases} 
\end{equation}
where $g(i,j)$ is the geodesic distance between the viewport centres of 
users $i$ and $j$ and $G_{th}$ is thresholding value, introduced in Section II. 
% Note that the clique-based clustering algorithm that we present in the following gets in input  binary adjacency matrices. Hence, $\text{W}_t $ is binary.

 %Finally, $N(i) = \{ j\in \mathcal{V}|w(i,j) >0, \forall j \}$ is the set of nodes neighbours to $v$. 
Looking at the graphs over time $\{ \mathcal{G}_t\}_{t=1}^T$, we are interested in clustering users based on their trajectories within a time window of duration $T$.  
In other words, we are interested in identifying users that have similar behaviour over time. With this goal in mind, we derive an affinity matrix $\text{A}$ that will be the input to our clustering algorithm Similarly to other clusters of trajectories \cite{atev2010clustering}. Each element of $\text{A}$ is defined as following:
  \begin{equation}\label{eq:affinity}
	a(i,j) = \mathcal{I}_\tau	\left(\sum_{t=1}^T w_t(i,j) \right)
\end{equation}
where the function $\mathcal{I}_\tau(\cdot)$ is defined as $\mathcal{I}_\tau(x)=1$ if $x\geq \tau$   and $0$ otherwise. %This means that users are neighbours if they have a viewport overlap above threshold in $D$ instants over $T$.
The matrix A can be associated to a trajectory-based graph where two nodes $i$ and $j$ are neighbours only if the corresponding viewports have a significant overlap in $\tau$ instants over $T$, \ie $a(i,j) =1$. The more threshold $\tau$ approaches $T$, the more stringent the similarity condition.
%\noteSR{Not sure to have got your comment..So can I simplify deleting all the following: In particular, when $\tau=T$ we have $a(i,j) =  \mathcal{I}_T \left(\sum_{t} w_t(i,j) \right) = \prod_{t} W_t$. This means that users' viewport centers need to be \emph{always} at a distance below threshold $\mathcal{G}_t$ to be neighbour. This condition is however too constraining especially in a trajectory context, therefore we have introduced the threshold value $\tau$.?}

\begin{figure}[t]
	\centering
%	\subfigure[Comparison pairwise geodesic distance and viewport overlap in Rollercoaster]{
%		\includegraphics[width=0.40\textwidth]{figures/GeodvsOver_Roller.eps}}
%	\subfigure[Timelapse]{
		\includegraphics[width=0.45\textwidth]{figures/ROC.eps} %}
	\caption{\ac{ROC} curve to evaluate optimal $G_{th}$ considering all video in database \cite{corbillon2017} and $O_{th}=80\%$ \label{fig:ROC} .} %The geodesic distance is plotted with inverse y axis making correspond low value of geodesic distance to high value of overlap.}
\end{figure}
\\
As clusters, we want to identify  group of users that are all neighbours (\ie $a(i,j)=1$ for all pairs of users $i$ and $j$ belonging to the cluster). In graph theory, a set of nodes that are all connected to each other is called a \emph{clique}. 
A clique perfectly matches with our definition of meaningful cluster: set of users all having significant pairwise viewport overlap, thus attending a common portion of video.
Therefore, we propose a \emph{clique-based clustering}.
%	To ensure that all users belonging to a cluster are attending the same area, they all need to be neighbors  % in a such way that all users belonging to the same cluster form a clique.
	  %Having clusters as cliques perfectly matches our application since % in the \ac{VR} context
 %While there is no a clustering methodology  where clusters are cliques (\emph{clique problem}), there are sub-optimal solutions related to  the clique problem. Here,
 In particular, we consider the \emph{Bron-Kerbosch (BK) algorithm} \cite{bron1973algorithm} to find all \textit{maximal cliques} present in our graph (\ie the most populated sub-graphs forming cliques). %Having clusters as much populated as possible would be beneficial in terms of future prediction.
	%However, maximal cliques identified by the BK algorithm can intersect, \ie 
While the BK algorithm identifies overlapping cliques (one user can belong to more than one clique), we are rather interested in identifying disjoint sets\footnote{Clusters should be disjoint for most content-delivery applications.
	For example, if clusters are used for prediction, each user must belong only to one cluster.}. %For this reason, the BK method cannot be  applied directly as clustering technique.
	Hence, we build upon the BK algorithm and propose a clustering algorithm aimed at identifying non overlapping cliques, as depicted in Fig.~\ref{fig:CliqueClustering}. % At the same time,  %Therefore, 
We initialize the clustering method by evaluating the affinity matrix from Eq.~\eqref{eq:affinity}. Then, we perform the following steps (Algorithm~\ref{Algorithm_CliqueCl}):
\begin{enumerate}
	\item Maximal cliques in the graph are detected by the BK algorithm. 
	\item  Among the resulting cliques, only the most populated one (with the highest cardinality) is kept as a cluster. % and added to the cluster variable $ \pmb{Q}$.  
	\item A new affinity matrix is built,  eliminating the entries corresponding to the elements of the cluster identified  in Step 2.
	\end{enumerate}
	These three steps are repeated until all nodes are assigned to clusters. It is worth mentioning that this iterative selection does not guarantee optimal clusters (\ie maximal joint overlap within the cluster). However, $i)$ it imposes viewport overlap among users within a cluster, $ii)$ it identifies highly populated clusters, which can be translated in reliable trajectories/behaviours shared among users. 
	
%%%%%
	\begin{figure}[t]
		\centering
		\includegraphics[width=0.4\textwidth]{figures/Clique_clustering.eps} 
		\caption{\label{fig:CliqueClustering} Graphical example of the proposed clique clustering.}
	\end{figure}
	 

 
	\begin{algorithm}[t]
	\begin{algorithmic} 
	%	\SetAlFnt{\small}
%		\SetAlCapFnt{\small}
%		\SetAlCapNameFnt{\small}
		%\algsetup{linenosize=\tiny}
		\caption{Clique-Based  Clustering }\label{Algorithm_CliqueCl}
  		%
		%\DontPrintSemicolon
		\STATE \textbf{Input:} \hspace{0.4cm} $\{ \mathcal{G}_t\}_{t=1}^T$, D\\
		\STATE\textbf{Output: } \hspace{0.07cm}$K, \pmb{Q} = [Q_1,...,Q_K]$  \\
		\STATE\textbf{Init: } \hspace{0.07cm}$i=1$, $\text{A}^{(1)}=\mathcal{I}_D(\sum_tW_t),  \pmb{Q}=[\{\emptyset\}, \ldots, \{\emptyset\}]$ \\
	  		 
		\Repeat{ $A^{(i)}$ is not empty  }{
			%Each point is assigned to the cluster with the closest centroids.
			\STATE  $\pmb{\mathcal{C}} = [\mathcal{C}_1,..., \mathcal{C}_{L}] \leftarrow   KB(\text{A}^{(i)})$ \\
 			\STATE   $l^{\star} =  \text{arg }\max_l |\mathcal{C}_l|$\\
 			\STATE  $ {Q}_i =   \mathcal{C}_{l^{\star}}$\\
			\STATE $\text{A}^{(i+1)} = \text{A}^{(i)}(\pmb{\mathcal{C}}  \setminus  \mathcal{C}_{l^{\star}})$
 			\STATE $i$ $\leftarrow$ $i+1$
		}
		\STATE $K=i-1$
		\end{algorithmic}
	 	\end{algorithm}
%%%%


==> ICASSP_2019/intro_3_SR.tex <==
\section{Introduction }        
%\textbf{[VR and AR becoming trendy: They involve new kind of visual signals, i.e., 360$^\circ$ videos]}\\
%In the near future, %\ac{AR} and 
%\ac{VR} systems are expected to become wide spread, with many applications (entertainment, e-healthcare, e-education, and many others).
\ac{VR} systems are expected to become wide spread in the near future, with applications spanning a variety of fields, from entertainment to e-healthcare. These systems involve omnidirectional ( \ie 360$^\circ$) videos, which are visual signals defined on a virtual sphere depicting the 360$^\circ$ surrounding scene. %\noteFDS{AR does not really invole 360 videos so I removed it}.
The viewer is virtually positioned at the centre of this sphere and can navigate the scene with three \ac{DOF}, \ie yaw, pitch and roll. The navigation is experienced by the user rotating his head and changing his viewing direction. This interactive navigation is typically enabled by a \ac{HMD}, which renders at each instant in time only the portion of the spherical content attended by the user, \ie \textit{viewport}. 

%\textbf{[navigation patterns analysis]}\\
Understanding how users explore the VR content is important in order to optimize content creation~\cite{Serrano2017} and distribution~\cite{rossi2017navigation,corbillon2017viewport,petrangeli2017http,fan2017fixation,Yu2015}, develop user-centric services~\cite{Broeck2017,Sitzmann2018}, and even for medical applications that use VR to study psychiatric disorders~\cite{srivastava2014virtual}. %, identifying individuals who show outlier behaviours~\cite{srivastava2014virtual}.
%
In the last few years, many studies have appeared collecting and analysing the navigation patterns of users watching VR content~\cite{Yu2015,Upenik2017,hu2017head,wu2017,corbillon2017,lo2017360,fremerey2018avtrack360, Singla2017,Sitzmann2018}. 
Most studies build content-dependent \textit{saliency maps} as main outcome of their analysis. The saliency map computes the most probable region of the sphere attended by the viewers, based on their head or eye movements~\cite{Duchowski2002, Yu2015, david:2018:DHE:3204949.3208139, Upenik2017, Rai2017}. Some studies also provide additional quantitative analysis based on metrics, such as the average angular velocity, frequency of fixation, and mean exploration angles%, \red{frames to reach the main attraction of the scene (i.e., \ac{RoI})}
~\cite{Sitzmann2018, corbillon2017}. %, percentage of fixations in a \ac{RoI}
%Models to predict future saliency maps have also been proposed~\cite{Bogdanova2008,Bogdanova2010,xu2017modeling}.\noteSR{Are so relevant to cite? Seems to interrupt the flow...because we were talking about quantitative metric, then we talk about prediction and again quantitative metric..}
However, none of these studies provide a quantitative metric to evaluate common patterns. On the contrary, performing a clustering of navigation trajectories can show how many groups of users consistently share a similar viewport over time. The evaluation of common portion (\ie overlapped viewport) of 360$^\circ$ content among users could be a key-metric to evaluate users' behaviour. This information might be useful in order to improve the accuracy and robustness of algorithms  predicting users navigation paths. A proper clustering could also be useful to refine user-centric distribution strategies, where for instance different groups of users might be served with higher quality content in different portions of the sphere  that will be more likely displayed by the viewers.  In this context, the main goal of this paper is to propose a novel clustering strategy able to detect meaningful clusters on the spherical domain. %we argue that, in 360$^\circ$ content,
%where 
We consider as meaningful cluster a set of users \emph{attending the same portion of spherical content}. \ie a set of users with substantial overlap between viewports. The main motivation is that a significant common overlap needs to be guaranteed for clustering methods to be used for prediction purposes or for implementing accurate user-based delivery strategies.

To the best of our knowledge,  studies identifying clusters for omnidirectional content delivery have appeared only recently \cite{xie2018cls,Gwendal2018}. User clustering is employed to identify the number of \acp{RoI} over time and to perform long-term trajectory prediction. In \cite{xie2018cls}, the viewing directions of each user at each instant in time, \ie viewport centers, are considered as points on the equirectangular planar. These are then clustered based on Euclidean distance, neglecting the actual spherical geometry. Conversely, in~\cite{Gwendal2018} %clustering of trajectories is performed taking into account the spherical domain, namely
each user navigation pattern is modelled as independent trajectories in roll, pitch, and yaw angles, %. Users are represented as center of their viewport
and spectral clustering is then applied. While it is efficient in discovering general trends of users' navigation, this clustering methodology is not focused on identifying clusters that are consistent in terms of overlap between viewports displayed by different users. This means that users in the same cluster do not necessarily consume the same portion of content. In other words, the identified clusters are not necessarily meaningful in the perspective of studying 360$^\circ$ navigation patterns.

In this paper, we propose a clique-based clustering to overcome the above limitations. First   we define a metric to %of similarity among users that
quantify the geometric overlap between two viewports on the sphere (Section II).
Then, we use this metric to build a graph whose nodes are the centers of the viewports associated to different users. Two nodes are connected only if the two corresponding viewports have a significant overlap (Section III). Finally, we propose a clustering method based on the Bron-Kerbosch (BK) algorithm \cite{bron1973algorithm} to identify clusters that are cliques, \ie sub-graphs of inter-connected nodes (Section III).  
Results demonstrate the consistency of the proposed clustering method in identifying clusters where the overlap between the portions of the spherical surface corresponding to different viewports is higher than in state-of-the-art clustering (Section IV). 
%Then, we extend traditional clustering techniques to spherical data and develop a clique-based clustering algorithm. Namely, we build a graph at each instant in time connecting the centroids of the viewports of users based on the similarity metric mentioned above.  Then, we impose the constraint that a cluster needs to be a  clique, i.e.,  sub-graphs of inter-connected nodes.  Cliques are identified by the Bron-Kerbosch (BK) algorithm \cite{bron1973algorithm}, and clusters are built starting from these cliques. Experimental results are carried out based on real-traces data set  with the clustering performed both at the frame-level (cluster of points) and over a time-window (cluster of trajectories).
%Results demonstrate the consistency of the proposed clustering method in identifying clusters where the geometric overlap between the portions of the spherical surface corresponding to different viewports is higher than state-of-the-art clustering.  
 % 
In summary, the main contribution of this paper is to propose a clustering algorithm that $i)$ considers the spherical geometry of the data, $ii)$ identifies clusters in which there is a consistent and significant %n actual 
geometric overlap between the portions of spherical surface corresponding to viewports attended by different users (by imposing that clusters are cliques), $iii)$ can be applied to a single frame or to a series of frames (trajectories). %, i.e., trajectory-based, clustering. %, $iv)$  introduces a constraints on the  geodesic distance to be  used as a proxy of viewport overlap. 
%\red{add potential/benefit? is that cool?}
This is a useful new tool to improve the accuracy of user's navigation prediction algorithms and user-dependent VR content delivery strategies, such as those proposed in~\cite{xie2018cls,Gwendal2018}.
%	We develop a novel methodology to analyse users’ behaviour with the final goal of answering to two basic and yet essential questions:\\
%	%1) Do users look at the same portion of the video content over time? and how much are they correlated based on their navigation on the sphere? \\
%	%2) \emph{How does a single user navigate within a given scene across time?} \\
%	1) Can we identify multiple sets of users who share the same navigation behaviour, i.e., look at the same portion of the spherical content at each instant in time and over a time segment? \\
%	2) Do these sets of users correlate with video content features?\\
%These clusters can be useful across different optimization tasks in the end-to-end delivery chain of \ac{VR} content.

%\textbf{[what is a cluster for us: a set of users whose FoV overlap for more than a threshold over a time window X]}\\
%\textbf{[We propose to use the clique to identify such clusters on a custom graph that we build]}\\
%Our goal is to propose a novel clustering strategy able to detect meaningful clusters in spherical domain, where a cluster groups the set of users whose viewports have a significant overlap on the sphere.
%display a portion of the sphere having an overlap over a defined threshold in a certain time window.
%We are not only interested in understanding if users are looking in similar directions. We are rather interested in understanding if users are displaying a significantly similar portion of the video within one frame or multiple frames. Specifically, we define a cluster as a set of users who display a portion of the sphere having an overlap over a defined threshold in a certain time window.

%\textbf{[Structure]}\\
%The reminder of this paper is organized as follows.  In Section II, we define the metric of similarity among users that we use to identify geometric overlap of viewports. 
%In Section III, we describe our clustering method based on a maximal cliques algorithm. Finally, in Section IV  we provide simulation results to demonstrate the consistency of the proposed clustering method in identifying clusters with high viewport overlap and we provide  conclusions and future works in Section V. 



% . First, we build a graph connecting the centroids of the viewports of all users at each instant in time, based on the similarity metric mentioned above. Then, we identify clusters as cliques, i.e.,  sub-graphs of inter-connected nodes, based on the Ken-Borchon clique detection algorithm [add ref]. In Section III, experimental results 
%We proposed to use an important proprieties of graph theory such as \textit{complete sub-graphs} or \textit{cliques} \cite{fortunato2010community}, to identify clusters in a customise graph based on the previous metric. 

%\textbf{[paper structure]}\\
% In the following as first step, we first define a novel sphere-based metric. Then we % extend traditional clustering techniques to spherical data and
%propose a clique-based clustering algorithm. Finally, we provide simulation results to validate the consistency of the clustering method and compare it to traditional clustering solutions. 



%%%%%%%%%%%%%%%

%[visual attention in VR]\\
%
%In \cite{Duchowski2002} a method for the comparison of human and artificial scanpaths recorded in VR is proposed and evaluated. The comparison method is based on the well-known scanpath similarity indices derived from string editing, successfully used to measure the accuracy of visual attention models over still images. %Scanpath similarity indices have successfully been used to measure the accuracy of visual attention models over still images. 
%An attentional model previously used for view-dependent enhancement of Virtual Reality is evaluated. [check details]
%% Modeling visual attention in VR: Measuring the accuracy of predicted scanpaths. Ph.D. Dissertation. Clemson University.
%% http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.91.5486&rep=rep1&type=pdf
%
%In \cite{Bogdanova2008} and \cite{Bogdanova2010} bottom-up methods to obtain saliency maps from omnidirectional images for static and dynamic cases are proposed. Features are computed and fused in a spherical domain. However, these studies do not provide any detailed descriptions about interpretation of experimental visual attention data for omnidirectional images. [check details] \\
%%[6] I. Bogdanova, A. Bur, and H. Hu ̈gli, “Visual attention on the sphere,” IEEE Transactions on Image Processing, vol. 17, no. 11, pp. 2000–2014, 2008
%%[7] I. Bogdanova, A. Bur, H. Hu ̈gli, and P.-A. Farine, “Dy- namic visual attention on the sphere,” Computer Vision and Image Understanding, vol. 114, no. 1, pp. 100–110, 2010.

%[pixel viewing probability in VR]\\
%
%In \cite{Yu2015}, the attended viewport at each instant in time is used to compute the pixel viewing probability, i.e., the relative frequency at which each pixel on the equirectangular grid is in the field of view of the user, averaged over time and all user set. %It is assumed that all points of the viewport are attended.
%This results in a heat map that collapses the temporal dimension, used to weight pixel-based distortion measures to compare the visual quality of 360-degree content undergoing different sphere to plane projections. \\
%, assuming that distortions affecting in the most attended part of the sphere have a stronger impact on the visual quality perceived by the user. 
%
%Peak accesses happen near %φ = ±30% since uniform sampling on viewport positions results in a denser access of points on the sphere as we move away from the equator.
% MattYu,HaricharanLakshman,andBerndGirod.2015.AFrameworktoEvaluate Omnidirectional Video Coding Schemes. In 2015 IEEE International Symposium on Mixed and Augmented Reality. 31?36.
%We use the head motion data to train two types of statistics on the sphere:
%- Relativefrequencyofaccessingdifferentpointsonthesphere according to viewing probabilities. This is visualized as a heat map in Fig. 5a.
%- Relative frequency of latitude-wise accesses, to succinctly capture the underlying dynamics, as shown in Fig. 5b.
%that peak accesses happen near %φ = ±30◦ since uniform sampling on viewport positions results in a denser access of points on the sphere as we move away from the equator.

%[head movements as proxy for eye movements in VR]\\
%
%% Evgeniy Upenik and Touradj Ebrahimi. 2017. A simple method to obtain vi- sual attention data in head mounted virtual reality. In 2017 IEEE International Conference on Multimedia & Expo Workshops (ICMEW). 73?78.
%In \cite{Upenik2017}, %a method is proposed to derive gaze fixation maps from head trajectories of users navigating 360-degree images.
%the head position at each instant in time, identified by the coordinates of the center of the viewport attended by the user, is used to approximate the gaze fixation. Data from different users are fused based on spatial proximity (not clear if euclidean or geodesic distance is used). A Gaussian distribution of eye fixations around the center of the viewport is assumed, as usually done in literature to produce saliency maps for viewing of 2D images. Therefore, a Gaussian kernel, adapted to account for the warping caused by the equirectangular projection, is used to produce continuous fixation maps. In this approach, not all the pixels of the viewport participates to the same extent to the heatmap. 

% Upenik et al. [1] have also reported saliency maps obtained from head motion tracking by assuming that the focus of interest is concentrated in the center of a given view-port, and applying a gaussian kernel as in usual saliency map design for 2D images to mimic the foveation filter. Consequently, as opposed to Yu et al [2], not all the pixels of the view- port participates to the same extent to the heatmap, which seems a more reasonable hypothesis considering the field of view offered by current HMDs.

% we assumed a Gaussian distribution of eye fixations around the center of a viewport.
%As conventional images typically a Gaussian filter is applied to model human acuity vision region of 1-2 degrees
%In case of head direction fixations the authors assume that the region of possible attention is 30 degrees.
%
%A gaussian filter kernel adapted to the equirectangular projection is proposed.
%
%We apply the proposed approach to compute fixation loca- tions and continuous fixation maps as interpretation of the raw experimental data described in Section 2. A head angu- lar velocity threshold equal to 15 degrees per second is used. The Gaussian filtering is performed using σ = 15 in the base function. In order to fuse individual fixation locations, the points are summed up in cells of 1×1 degree. The modified Gaussian kernel Gmod(x,y) is used to filter the data in the equirectangular domain. Figure 5 shows the fixation locations and the continuous fixation maps for four contents used in the experiment.
%
%The head position at each instant in time is approximated by the coordinates of the center of the viewport visualized at that instant in time. % Raw data of a head direction trajectory contains an array of yaw and pitch coordinates along with their time-stamps. 
%Observer head position is identified by the yaw and pitch values associated to the center of the viewport. %The head angular velocity is computed a first order derivative of the yaw and pitch values.
%The head angular speed %(first order derivative of the yaw and pitch values)
%is used to exclude the parts of a trajectory where motion is too fast to fixate viewer's attention. % we assume there exits a threshold head angular velocity beyond which users are not able to focus their attention on any object. The value of 15 degrees per second has been chosen as the upper boundary for this paper. 
%
%Fixations of different subjects are fused together by summing-up all the points in cells with specified size on the yaw-pitch plane. % producing a weighted set. %If needed, this step is preceded by re-sampling track coordinates in order to conform to the equal distribution of points on a sphere.
%
%Finally, a Gaussian based filtering is performed to produce continuous fixation maps. %Fixation location data does not typically allow to properly depict the regions of visual attention. Because of its discrete nature, this information is not consistent even among human subjects.
%Indeed, very rarely a person will fixate their attention in the same exact point as another. %Thus there is a need to introduce a statistical areas of fixations.
%For conventional images typically a Gaussian filter is applied to model human acuity vision region of 1-2 degrees.
%In case of head direction fixations the authors assume that the region of possible attention is 30 degrees.
%
%A gaussian filter kernel adapted to the equirectangular projection is proposed.
%
%We apply the proposed approach to compute fixation loca- tions and continuous fixation maps as interpretation of the raw experimental data described in Section 2. A head angu- lar velocity threshold equal to 15 degrees per second is used. The Gaussian filtering is performed using σ = 15 in the base function. In order to fuse individual fixation locations, the points are summed up in cells of 1×1 degree. The modified Gaussian kernel Gmod(x,y) is used to filter the data in the equirectangular domain. Figure 5 shows the fixation locations and the continuous fixation maps for four contents used in the experiment.

%In \cite{Rai2017}, 
%% eye movements analysis has proved to provide an important added value to visual attention modeling in VR [16]
%% YashasRai,PatrickLeCallet,andPhilippeGuillotel.2017.Whichsaliencyweight- ing for omni directional image quality assessment?. In Quality of Multimedia Experience (QoMEX), 2017 Ninth International Conference on. IEEE, 1?6.
%eye-gaze data is analysed to verify whether eye gaze saliency can be approximated by head motion saliency for navigation of 360-images.
%% It is mentioned that, due to the fact that an equirectangular projection is neither equi-area nor conformal, and several other panorama formats like cube- maps suffer from problems of border-discontinuity,
%To distinguish between fixations and saccades, the orthodromic distance between gaze points on the spherical surface is computed, divided by time. % reflects the velocity of gaze movement that can be used to classify the gaze data into fixations and saccades. % either based on a velocity or based on a dispersion algorithm.
%A Gaussian filter of two degrees visual angle centered at each fixation point is then applied. % on the viewport plabe, in order to spread the fixations within the viewport plane.
%The Gaussian filtering is applied in the viewport space because it is this image that was visible to the observer within the HMD. The resulting image is projected into the equirectangular domain to produce the heatmap. % to reflect the effect of the current fixation.
%A similar technique is applied to all fixations, from all observers and the equirectangular-map is updated each time with the sum.
%% comparing heatmaps
%A method to compare multiple heatmaps is also proposed, based on uniform resampling of the data in spherical domain. \\
%%Two equirectangular saliency maps cannot be compared directly like two-dimensional saliency maps, because the poles of the sphere are over represented at the equirectangular image top and bottom ends.
%%Elliptical sampling [6] is used to generate uniform sampling points on the sphere. These points are projected into the equirectangular image, so that the saliency values at these points can be sampled.
%
%Analysis of the offset between the center of the rectilinear view-port image and the point of fixation (henceforth referred to as relative gaze offset)
%- the region that the observers usually look at is not the center of the rectilinear image: but is instead offset from the center by about 12 degrees. Consequently, one should be cautious when applying gaussian weighting (especially its standard deviation, which is usually 2-degree centered on the view-port to mimic the foveation filter.
%
%Comparison of the saliency maps that are a result of the head and eye based attention data, versus that resulting from head movement data alone
%%- Viewport uniform (head motion data only): Uniform weighting in the viewport also referred to as Frequency of pixel access from head-movement analysis by [2], considers that the entire rectilinear image visible in the view-port is salient at a given time instant. It weights far peripheral areas the same as the foveal ones.
%%- Viewport gaussian method (head motion data only) consists of applying such a Gaussian weighing centered at the middle of the rectilinear(viewport) image. 
%%- Eye-centered Gaussian method applies the same Gaussian weighting, but on the actual eye(plus head) positions of the observers in the experiment.
%%- Viewport ProbMap method (Head motion only). It consists of applying the probability distribution represented in Figure 4 instead of the Gaussian, for weighing the view-port rectilinear image
%
%KL divergence to compare maps

%[consumption-experience of 360 videos in VR]\\
%
%\cite{Broeck2017}
%%% It?s All Around You: Exploring 360-degree Video Viewing Experiences on Mobile Devices (ACM MM 2017)
%%%observed 18 participants? interaction with six 360° videos with different viewport characteristics (static or mov- ing) on a smartphone, a tablet and a head mounted display (HMD) respectively and measured how they interact with the content.
%%%i) How di erent viewport characteristics of a 360° video in uence viewers? behaviour
%%%we quantitatively logged 18 users? exploration patterns on a smartphone, a tablet and an HMD respectively while watch- ing six 360° videos produced with both static viewport (SVP) or moving viewport (MVP)
%%%MVP videos, no matter what content was shown, consistently require more exploration from viewers than SVP videos for all three devices. On average, all participant?s exploration rate with MVP videos was 17.3° per 30 seconds, on the contrary for SVP it was 14.6° per 30 seconds. We run a paired samples t-test to evaluate the di erence in the exploration rate on viewports across all partici- pants and found signi cant di erence in the exploration rate for SVP and MVP (t (53) = ?12.933 and p < .01).
%%%Plots: exploration as the degree of user activity of looking around in the 360° video to dis- cover more content.
%%%We notice that SVP videos typically have an initial exploration phase, in contrast MVP videos are explored throughout.?> SVP = one or multiple static viewports (i.e. the cameras were placed on a stand in the centre of the scene to record the 360° video ), MVP = used moving viewports (i.e. the cameras were moved while recording the video).: viewers explore the viewports as they keep changing instead of focusing on the moving action frame.
%%% SVP videos elicit explo- ration in short bursts followed by a short period of no exploration.
%
%\cite{Serrano2017}
%% Ana Serrano, Vincent Sitzmann, Jaime Ruiz-Borau, Gordon Wetzstein, Diego Gutierrez, and Belen Masia. 2017. Movie editing and cognitive event segmentation in virtual reality video. ACM Transactions on Graphics (TOG) 36, 4 (2017), 47.
%% Serrano et al. used head and eye tracking data for movie editing and segmentation [19]
%
%\cite{Su2016} \\
%%Yu-Chuan Su, Dinesh Jayaraman, and Kristen Grauman. 2016. Pano2Vid: Automatic Cinematography for Watching 360? Videos. 1 (Dec. 2016).
%%Su et al. [21] used head movements for automatic cinematography in 360 videos. \\

%[360 image navigation datasets and analysis]\\
%
%\cite{Rai20171}
%% A dataset of head and eye movements for 360 degree images.
%% https://doi.org/10.1145/3083187.3083218
%
%\cite{Hu2017} \\
%%Brian Hu, Ishmael Johnson-Bey, Mansi Sharma, and Ernst Niebur. 2017. Head movements during visual exploration of natural images in virtual reality. In 2017 51st Annual Conference on Information Sciences and Systems (CISS). 1?6. https://doi.org/10.1109/CISS.2017.7926138

%[360 video navigation databases and analysis]\\
%
% \cite{Wu2017}
%%A Dataset for Exploring User Behaviors in VR Spherical Video Streaming
%% analyse exploring behaviors based on head tracking data for video streaming of omnidirectional video [23]
%
%\cite{Corbillon2017}
%% Xavier Corbillon, Francesca De Simone, and Gwendal Simon. 2017. 360-Degree Video Head Movement Dataset. Proceedings of the 8th ACM on Multimedia Systems Conference - MMSys?17 (June 2017), 199?204.
%
%\cite{Lo2017} \\
%% 360 Video Viewing Dataset in Head-Mounted Virtual Reality. In Proceedings of the 8th ACM on Multimedia Systems Conference. ACM, 211–216.
%%the 360-degree video viewing dataset in head-mounted VR, by Lo et al. [10] (ten videos from Youtube, duration of one minute, watched by 50 users)
%
%% the dataset for emotion induction research by Li et al. [9] containing head movement data and corresponding ratings of arousal and valence (73 videos from Youtube, durations from 29 to 668 seconds, watched by 95 users) \\
 
% [streaming]\\
 
% \cite{Fan2017}
%% Ching-LingFan,JeanLee,Wen-ChihLo,Chun-YingHuang,Kuan-TaChen,and Cheng-Hsin Hsu. 2017. Fixation Prediction for 360 Video Streaming in Head- Mounted Virtual Reality. In Proceedings of the 27th Workshop on Network and
%% Operating Systems Support for Digital Audio and Video. ACM, 67–72.
% 
% % application of head movements for e cient delivery of 360-degree video
%% Xavier Corbillon, Gwendal Simon, Alisa Devlic, and Jacob Chakareski. 2017. Viewport-adaptive navigable 360-degree video delivery. IEEE International Con- ference on Communications (2017).
%
% \cite{Singla2017} 
% 
%% \cite{Sitzmann2018}
%% % SALIENCY IN VR: HOW DO PEOPLE EXPLORE VIRTUAL ENVIRONMENTS? | IEEE VR 2018
%% % https://doi.org/10.1109/TVCG.2018.2793599
%
%% 360-Degree Video Streaming and its Subjective Quality
% \cite{Curcio2017} \\
 
% [prediction]
% 
% \cite{Xu2017} \\
%% Mai Xu, Yuhang Song, Jianyi Wang, Minglang Qiao, Liangyu Huo, and Zulin Wang. 2017. Modeling Attention in Panoramic Video: A Deep Reinforcement Learning Approach. arXiv preprint arXiv:1710.10755 (2017).
 
% [MMSys 2018 - datasets]  \\
% 
%% % A Dataset of Head and Eye Movements for 360-degree Videos
%% \cite{David2018}
%%%a dataset of videos containing head and eye tracking data for research on exploring behaviors with 360? dynamic content. The dataset contains 19 videos in equirect- angular format with associated data of head and eye movements collected from a free-viewing experiment with 57 observers wear- ing a VR headset with an integrated eye-tracker. In addition, we analyze users? exploring behavior such as the impact of starting longitudinal positions on 360? content exploration, and the relation between head and eye movement data.
% 
%  \cite{Fremerey2018}
%  % AVTrack360: An open Dataset and So ware recording people?s Head Rotations watching 360? Videos on an HMD
  
  
  %%%%%%%%%%%%%%
%
%\noteFDS{DA QUI IN POI E' VERSIONE PRECENDENTE CHE E' ANCHE OK MA TROPPO LUNGA :( DI BASE HO CERCATO DI RIASSUMERE TUTTO. BISOGNA CONTROLLARE REFERENCE - HO AGGOUNTO BIB FILE CHE AVEVAMO FATTO PRECENDENTEMENTE MA NON TUTTO FUNZIONA}
%
%In these user-centric services, it is essential to study, analyze and understand how users visually explore the VR content. In the context of interactive communications, the  ultra   high spatio-temporal resolution of 360-degree videos, the low latency required to provide real VR experiences, as well as the novel interacting way of consuming this media have raised novel compelling challenges, that could benefit from users' prediction. Tile-based encoder could optimize the tiles design based on the users navigation [xx]. Service providers, that  need to store different versions (different coding and resolution parameters) of one video content in DASH streaming, could reduce their storage costs keeping only the representations that will be of interested for the users [XX].  Finally, the prediction of users navigation could substantially improve the delivery of omnidirectional videos if  the content of most likely displayed by the user is prioritized (viewport-aware streaming \cite{rossi2017navigation,corbillon2017viewport,petrangeli2017http}).  %Hence, the need to analyze, study and predict interacting users.  
%Beyond communications, in  the medical context,   VR has been considered a major tool for investigation,  of medical and psychiatric disorder \footnote{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC4361984/.}%\footnote{https://www.kcl.ac.uk/ioppn/depts/psychology/research/researchgroupings/vrrg/projects-at-the-virtual-reality-research-group.aspx}. 
%This has been possible by understanding the interaction of the user with the content.  \noteLT{not sure if we wanna also say that as shown with eye-gazing, understanding user behavior has many potentiality.}
%%
%In summary,   predicting how people navigate within the omnidirectional content is a key-factor to unlock  \ac{VR} communications and services at large. 
%    Hence, the increasing interest in the field of users' behaviour prediction and analysis. While many recent works have been focused on the prediction of saliency map (density of users watching in a given direction at a given time) for 360 images, saliency for 360 videos as well as the actual prediction of navigation patterns (sequential directions watched by one user in time) for 360 content is still overlooked. To achieve an accurate prediction, there is the need to study and understand the interactive behaviour of users. Several datasets have been made available to support this emerging research area, and data analysis is proposed for most of the datasets. Used metrics are visual attention map (frequency of fixation in terms of elevation and azimut) \footnote{?Modeling Visual Attention in VR: Measuring the Accuracy of Predicted Scanpaths,? in Eurographics 2002 - Short Presentations. Eurographics Association, 2002.}\footnote{?360-degreee video head movement dataset,? in Proceedings of the 8th ACM on Multimedia Systems Conference, ser. MMSys?17.}, mean exploration angles \footnote{?It?s all around you: Exploring 360-degree video viewing experiences on mobile devices,? in Proceedings of the 2017 ACM on Multimedia Conference, ser. MM ?17. New York, NY, USA: ACM, 2017}, frames to reach ROI (region of interest), percentage of total fixations in the ROI, scanpath error between each user and a dominant scanpath \footnote{Saliency in VR: How do people explore virtual environments?? IEEE Transactions on Visualization and Computer Graphics, vol. 24, no. 4, pp. 1633?1642, April 2018. [5]: ?A dataset of head and eye movements for 360 degree images,? in Proceedings of the 8th ACM on Multimedia Systems Conference, MMSys?17.}, angular distance between user positions in a temporal window \footnote{David-LaCallet MMSys 2018}, estimation of gaza velocity, head trajectory, gaza and head scanpath\footnote{?Visualization and analysis of head movement and gaze data for immersive video in head-mounted displays." In Proceedings of the Workshop on Eye Tracking and Visualization (ETVIS), vol. 1. 2015.}. But, how do we make sense out of these data and metrics? All the above metrics are useful but none of them can answer one simple question: are users predictable? Developing an efficient tool for navigation patterns analysis in the spherical domain and leverage on that to predict users behaviour is the.
% 
%Quindi un bisogno imminente di sviluppare proper frameworks per studiare gli utenti. Molte ricerche son state fatte gia? in questa direzione MA
%- molti laovri di saliency lavorano sul planar direttamente. 
%- quelli che sono adattati sulla sfera comunque offrona un?accurate saliency che pero? offre solo una partial visione del comportamento degli utenti (qualitativamente come sono focalizzati ma non quando sono simili o come si muovono nel tempo). 
%- il movimento puo? esser studiato con velocita? angolare per esempio ma questo non permette pero? di capire effettivamente la similitudine tra utenti (due utenti possono avere la stessa velocita? angolare nel tempo ma puntare in due direzioni diverse). 
%- extensive data set sono stati creati e questo favorische futuri studi nella topic. Alcuni hanno anche procurato un analisi del dataset ma di solito con molte metriche invece che una unica. 
%
%- una promising solution e; di considerare il clustering. Permette di accomunare utenti in base ai loro comportamenti in un istante (dove guardano ora?) or in una finestra temporale (utentti interagiscono col contenuto enllo stesso modo). temporal clustering if properly done permette anche una prediction temporale come gwendal. therefore, we focus on the clustering as possible metric to provide global view of the users bevaior (possiamo anche dire che il K vs time ci permette anche di capire il FOA etc). 
%
%- however, non e; chiaro cosa significhi un meaningful cluster in VR e parliamo dell?overalp etc. 
%
% 
%
%%	To optimise the storage, consumption such as the delivery of omnidirectional video is then essential study how users visually explore this content. %In fact% the final quality perceived by the user is strongly affected by the displayed content \cite{rossi2017navigation}. 
%%	Viewport-aware streaming strategies have been proposed in order to privilege the area that most probably will be displayed by users \cite{rossi2017navigation,corbillon2017viewport,petrangeli2017http}.  \\
%	%%%%%%%%%%%%%%%%%%\textbf{[mention what are the existing works on analysis of navigation of 360-degree content]}\\
%
%. A general statistical characterization of users' behaviour has been presented with new publicly available 360$^\circ$ image and video datasets with user tracking data  \cite{corbillon2017,lo2017360,wu2017,hu2017head,rai20171,fremerey2018avtrack360,david:2018:DHE:3204949.3208139}. 
%\noteLT{maybe we could say that general behaviors have been deduced, for example that users are always more scattered at the beginning of the video etc. } However, this characterization is usually performed via a set of multiple-metrics (e.g, angular velocity, content spanned over time, head direction)  that not with one global metric able to reflect the actual behavior of the  users and that could be directly adopted into optimization frameworks.  
%%%%%%%%%%%	\textbf{[What is missing in these studies? problems with analysis on equirect domain; qualitative analysis via heat maps not easy to provide quantitative indexes, especially when temporal axes is there; we are not aware of any clustering algorthim for 360 navigation patterns analysis. Clustering for eye tracking could be applied but 1) they are mostly for planar data (i.e. 2D image) 2) existing clustering does not account for the FoV overlapping, but only clusters points in space]} \\%prediction models depending on availability training data and complex to be implemented at client side]}\\	
%A compact metric to identify users behavior is the saliency map that  models the visual attention for omnidirectional video contents. Few works extend the state-of-the-art saliency map prediction algorithms to omnidirectional content \cite{deabreu2017look, monroy2018salnet360}. \noteLT{Is 11 really considering the spherical aspects? There is also this work if I'm not mistaken (Modeling Attention in Panoramic Video: A Deep Reinforcement Learning Approach) and there was also one from Patrick. }
%However, a saliency map models the attention of users within one single frame for a time window of the video content. This static analysis provides a key information, which is the per-frame attention of the users, but it does not provide information about the more dynamic behavior of users navigating over time. This dynamic behaviour is essential for tasks that need to predict where one single user will be looking at in the future, such as user-based adaptation logic algorithms. 
%\noteLT{I think we have to be careful here. Do we wanna sell our clustering for prediction purposes only? Not sure as we might not include the temporal aspect right? }
%\noteLT{There are some recent works on prediction (as the ones mentioned in gwendal's paper, I think we should include them. An option is to say that these ones do not provide accurate prediction, while clustering could do (as shown in gwendal's work) and we refer to the paper also for prediction in general}
%
%
%Clustering analysis is a traditional approach used to understand visual behaviours of people looking at multimedia content, i.e., images [ ], and to detect saliency area in a web page \cite{he2017graph}. Traditional cluster methods cannot be directly applied to omnidirectional content since they are mostly for planar data (i.e., 2D image). Moreover, they consider only the point location in the space without taking account for the overlapped displayed portion among elements in the same cluster. 
%	%In the literature, most of the works have been focused on predicting the saliency map, i.e., predicting the attention of users within one single frame []. This static analysis provides a key information, which is the per-frame attention of the users, but it does not provide information about the more dynamic behaviour of users navigating over time. This dynamic behaviour is essential for tasks that need to predict where one single user will be looking at in the future. User-based adaptation logic algorithms are an example of these tasks. However, despite its importance, the prediction of users’ navigation path has been overlooked.
%	
%	%        [In this paper:\\
%	%       Main contribution: we propose a new method to identify how many clusters exist of users who look at the same portion of sphere at a certain instant in time or over a certain time window.\\
%	%	How can this info be used?
%	%	\begin{itemize}
%	%	\item If too many clusters exist and they are not consistent over time, than this is a quantitative objective indicator that the prediction of user's patterns over a content (or a specific portion of it) might be challenging.
%	%	\item If clusters exist and are consistent over time, this info can be extracted by the video provider and: \\
%	%	-  shared with the client to facilitate his/her prediction. Particularly, in a DASH-like VoD video delivery session, if the client knows that his/her navigation has been consistent with that of a set of users on the first x seconds of a video sequence, he/she can use this information to select what segments to request for the future, assuming that he/she will likely continue to navigate the video as the set of users did. The prediction at client side will not be absed only on the user own navigation behaviour (is the user not moving his head at all or too much) but also on the behaviour of other users who watched the content before him/her.\\
%	%	- used to filter the segments to be pushed on edge servers, if the users served by the server show to have navigation paths that belong to some clusters.
%	%	\end{itemize}
%	%        An example application of how to use the quantitative data extracted using our method in a DASH VoD video streaming scenario is demonstrated.]\\ % where relevant amount of navigation patterns data is available to the service provider and the server can help the client to decide whether a prediction is possible or risky.]\\
%	
%		\textbf{[Contribution in this paper: we propose a new method to identify how many clusters exist of users who look at the same portion of sphere at a certain instant in time or over a certain time window.]}\\
%	In this paper, we propose a new method to identify how many clusters exist of users who look at the same portion of sphere at a certain instant in time or over a certain time window.
%	We develop a novel methodology to analyse users’ behaviour with the final goal of answering to two basic and yet essential questions:\\
%	%1) Do users look at the same portion of the video content over time? and how much are they correlated based on their navigation on the sphere? \\
%	%2) \emph{How does a single user navigate within a given scene across time?} \\
%	1) Can we identify multiple sets of users who share the same navigation behaviour, i.e., look at the same portion of the spherical content at each instant in time and over a time segment? \\
%	2) Do these sets of users correlate with video content features?\\
%These clusters can be useful across different optimization tasks in the end-to-end delivery chain of \ac{VR} content.
%
%\textbf{[what is a cluster for us: a set of users whose FoV overlap for more than a threshold over a time window X]}\\
%\textbf{[We propose to use the clique to identify such clusters on a custom graph that we build]}\\
%Our goal is to propose a novel clustering strategy able to detect meaningful clusters in the spherical domain. We are not only interested in understanding if users are looking in similar directions. We are rather interested in understanding if users are displaying the same portion of the video within one frame. Specifically, we define a cluster as a set of users who display a portion of the sphere having an overlap over a defined threshold in a certain time window. The key challenge is to define the proper metric that defines similarities among users in terms of this overlap. In particular, we proposed to use an important proprieties of graph theory such as \textit{complete sub-graphs} or \textit{cliques} \cite{fortunato2010community}, to identify clusters in a customise graph based on the previous metric. 

 

==> ICASSP_2019/results.tex <==


%%%%%%%%%%%%%%
\section{Experimental results}
%\textbf{[comparison with Louvain et K-mean]}
The proposed clustering algorithm is compared to state-of-the-art solutions, namely the \emph{Louvain method}  \cite{blondel2008fast}, the  \emph{K-means clustering} \cite{hartigan1979algorithm} and the clustering of \ac{VR} trajectories proposed in \cite{Gwendal2018} (labelled ``SC").  %To achieve a fair comparison,
We use the geodesic distance between viewport centers as distance metric in all algorithms.
Moreover, in the  \emph{K-means clustering}, the number of clusters $K$ is imposed as the value achieved by the Louvain method (labelled ``K-means 1"), as well as the $K$ value obtained from our proposed clustering  (labelled ``K-means 2"). The proposed implementations have been made publicly available~\footnote{{https://github.com/LASP-UCL/spherical-clustering-in-VR-content}.}.
% In \cite{Gwendal2018},  an affinity metric based on the users' trajectories is evaluated taking  into account the spherical geometry and neighbours between trajectories within a time interval $T_l = 2s$. This affinity matrix is the input to a spectral clustering \cite{atev2010clustering}.
 We test these algorithms on two  video sequences 1-minute long (Rollercoaster and Timelapse), which have been watched  by $59$ users whose navigation paths are publicly available~\cite{corbillon2017}. Rollercoaster has one main \ac{RoI} (i.e., the rail) while in Timelapse, there are many fast moving objects (e.g., buildings, people) along the equator line. %These videos are $1$ minute long and have been watched
 %, Rollercoaster and Timelapse, with navigation paths derived from a public dataset %(1 minute long, 30frame/sec and watched by 59 users) 
%\cite{corbillon2017}. %\red{ \noteSR{check if we've already said it in section 2!}}
%In the first case, , as well as the simple   based on the geodesic distance. 
%\textbf{[small decsription of  louvain method - maybe not needed as it is state fo the art. Highlight difference wrt proposed clique based approach, ie. it does not account for our definition of cluster]}\\
%The \emph{Louvain method} is one of the most popular unsupervised technique  to identify clusters in a graph \cite{blondel2008fast}. The main strengths of this algorithm are: simple to implement, automatically evaluates the number of clusters, and yet it is efficient. This makes it suitable also for large networks. This method is a greedy algorithm and is based on a density metric of clusters \cite{fortunato2010community}.
%that optimizes the \emph{modularity} in a graph . \emph{Modularity} is a metric to measure the density of clusters.
%\textbf{[small description of spherical K-means]}\\
%We also compare our results to the results of a modified version of the well-known and simple K-means algorithm, \emph{Spherical K-means clustering} that takes into account the spherical geometry of \ac{VR} content.  

{\textbf{Frame-based Clustering.}}
First, we consider frame-based clustering, in which users are identified by their viewport centers in one given frame. Table \ref{table} reports results in terms of number of clusters ($K$), mean viewport overlap computed within each cluster composed by at least three users, and viewport overlap within the most populated cluster, that we refer to as the main cluster. The viewport overlap within a cluster is the joint overlap across all users' viewports in the cluster. The mean overlap is computed by averaging the viewport overlap of all clusters with at least three users identified at a given frame. % the cluster overlap averaged over all clusters evaluated at a given frame and then averaged over time.
In Table \ref{table}, we also provide %the mean overlap calculated only for clusters with at least three users, as well as 
the percentage of users covered by clusters. The  proposed algorithm  always ensures the highest viewport overlap (on average always over 50\%) with respect to the other methods. This is due to the implicit constraint that is imposed by the clique-based detection of the clusters. This constraint leads to the identification of clusters that are populated and yet meaningful (i.e., with large viewport overlap among users). For example, in Rollercoaster at frame $40s$, our algorithm identifies a main cluster grouping $35\%$ of the population with a viewport overlap of $58.33\%$. This is much higher than the overlap of $24.20\%$ ($0\%$) in the main cluster identified by the Louvain (K-means) method. 
Beyond the accuracy, another important parameter is the percentage of %covered population, i.e.,
the population that is covered by clusters with a significant number of users. These clusters are the most useful ones to allow predictions.
% by clusters with at least $3$ users. %When used for prediction, for example, single-user clusters or very small clusters are not very \red{reliable}.
For instance in Timelapse at frame 50$s$, our method identifies a large number of clusters (29), which also includes single users clusters. % giving the possibility to have more small clusters.
Nevertheless, half of the population (51.70\%) belongs to clusters with more than $3$ users with high value of joint overlap (71.40\%). \par
 %Our algorithm detects more populated clusters with high values of joined overlapped viewports.}
%is still characterizes by no-single cluster with high value of joint overlap (71.40\%).
 %characterizes only part of the total population ($76.30\%$ in frame $40s$ of Rollercoaster as opposed to $100\%$ of K-Means $1$) but with more accuracy ($58.33\%$ overlap as opposed to $0\%$ of K-Means $1$). 
% The clustered population is lower than other algorithms but still acceptable. On the contrary, results from other techniques are more variable.
%To generalize results, we further extend the clustering analyse over time. Fig.~\ref{fig:AllVideo_OvInter_Var} (a) and (b) shows the mean and variance of the overall overlap over time for the frame-based algorithms considered in this work. 
%In more details, for each frame the optimal clusters are evaluated (based on one of the four algorithms). Then, the overall overlap is evaluated for each cluster. The mean and the variance per frame is finally provided in the figure. 
%Our proposed clique clustering is outperforming the others as it has the highest mean overlap and the lowest variance. This means that clusters obtained by the clique algorithm have always homogeneous and high value of overlap. For the other algorithms, instead, this feature is not ensured as already shown in Table\ref{table}. %In particular, in Rollercoaster the variance is very spread, as shown Figure~\ref{fig:AllVideo_OvInter_Var}.
% are firstly tested using the frame showed in Figure~\ref{fig:1_selected_frames}. %Figure~\ref{fig:RollerClustering}  visualise the clustering results for the frame 1480 of Rollercoaster. In these figures, the viewport centre of users belonging to the same cluster are plotted with identical colours. In addition, users alone in a cluster (i.e., isolated clusters) are plotted with a cross, to differentiate them from the populated clusters, marked with dots. Finally, clusters are also identified by their centroids with a red dot and a number, representing the cluster ID.
%\begin{figure}[t!]
%	\centering
%	\subfigure[Louvain Method]{
%		\includegraphics[width=0.23\textwidth]{figures/Roller_LouvainMethod.eps}}
%	\subfigure[Clique Clustering]{
%		\includegraphics[width=0.23\textwidth]{figures/Roller_Clique.eps}}\\
%	\subfigure[Spherical K-means Clustering 1]{
%		\includegraphics[width=0.23\textwidth]{figures/Roller_Kmeans1.eps}}
%	\subfigure[Spherical K-means Clustering 2]{
%		\includegraphics[width=0.23\textwidth]{figures/Roller_Kmeans2.eps}}
%	\caption{\label{fig:RollerClustering} Clustering results for Rollercoaster in Frame = 1480.}
%\end{figure}
%
%In the frame-example of Rollercoaster, the Louvain Method detects 8 clusters while the Clique clustering 12, Figure~\ref{fig:RollerClustering} (a) and Figure~\ref{fig:RollerClustering} (b), respectively. 
%As general trend, the second algorithm is more restrictive (leading to a greater number of clusters) as all users need to be neighbours to be gathered together within a cluster. For instance, the cluster n. 2 in Figure~\ref{fig:RollerClustering} (a) corresponds to 3 different clusters in Figure~\ref{fig:RollerClustering}(b), namely the clusters n. 3, n. 5, and n. 7. However, the extension of clusters is even bigger in the two K-means algorithms. Clusters n. 5 and n. 11 in Spherical K-means 1 and Spherical K-means 2 respectively are composed by the same users. However, it is evident that the overlap among users is not always high since they are very far. This means that users watching at different portions of the video content are erroneously gathered within the same cluster. \\
%To verify the efficacy of the Clique clusters, we consider the overall overlap within the cluster over time. This metric evaluates the percentage of overlapped viewports among all users in the same cluster. 

\begin{table*}[]
	\centering
	\resizebox{0.9\textwidth}{!}{%
		\begin{tabular}{cc||c|c|c|c||c|c|c|c|}
			\cline{3-10}
			&                                  & \multicolumn{4}{c|}{\textbf{ROLLERCOASTER}}                                                                                                                                                                                                                                                                                                          & \multicolumn{4}{c|}{\textbf{TIMELAPSE}}                                                                                                                                                                                                                                                                                                            \\ \cline{3-10} 
			&                                  & \textit{Louvain method}                                                                                & \textit{Clique Clustering }                                                                         & \textit{K-Means 1   }                                                                     & \textit{K-Means 2 }                                                                   & Louvain                                                                              & \textit{Clique Clustering }                                                                        & \textit{K-Means 1}                                                                      & \textit{K-Means 2}                                                                       \\ \hline
%			\multicolumn{1}{|c|}{\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Frame\\ 300\end{tabular}}}}  & K                                & 12                                                                                     & 23                                                                                  & 12                                                                                  & 23                                                                              & 15                                                                                   & 23                                                                                 & 15                                                                                & 23                                                                                 \\ \cline{2-10} 
%			\multicolumn{1}{|c|}{}                                                                               & Clusters(n. user \textgreater 3) & 5 (86.50 \%)                                                                           & 8 (64.50 \%)                                                                        & 7 (88.10 \%)                                                                        & 10 (62.71 \%)                                                                   & 7 (86.20\%)                                                                          & 13 (82.80\%)                                                                       & 9 (81 \%)                                                                         & 9 (65.50\%)                                                                        \\ \cline{2-10} 
%			\multicolumn{1}{|c|}{}                                                                               & Mean Overlap                     & 31.60 \%                                                                               & 71.90 \%                                                                            & 37 \%                                                                               & 55.80 \%                                                                        & 45.90\%                                                                              & 71.50\%                                                                            & 46.90\%                                                                           & 53.70\%                                                                            \\ \cline{2-10} 
%			\multicolumn{1}{|c|}{}                                                                               & Max pop cluster                  & \begin{tabular}[c]{@{}c@{}}1cl with 18u.\\ pop. 30.50\%\\ ov. 13.10\%\end{tabular}     & \begin{tabular}[c]{@{}c@{}}1cl. with 12u.\\ pop. 20.70\%\\ ov. 71.40\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}1cl. with 18u.\\ pop. 30.50\%\\ ov. 30.80\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}2cl. with 5u.\\ pop. 17\%\\ ov. 45.60\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}1cl with 15u\\ pop. 25.86\%\\ ov. 50.10\%\end{tabular}    & \begin{tabular}[c]{@{}c@{}}1cl with 9u\\ pop. 15.50\%\\ ov. 66.95\%\end{tabular}   & \begin{tabular}[c]{@{}c@{}}1 cl with 9u\\ pop 15.50\%\\ ov 26.95\%\end{tabular}   & \begin{tabular}[c]{@{}c@{}}1 cl with 9 u.\\ pop 15.50\%\\ ov. 0\%\end{tabular}     \\ \hline
%			\multicolumn{1}{|c|}{\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Frame\\ 600\end{tabular}}}}  & K                                & 14                                                                                     & 21                                                                                  & 14                                                                                  & 21                                                                              & 15                                                                                   & 26                                                                                 & 15                                                                                & 26                                                                                 \\ \cline{2-10} 
%			\multicolumn{1}{|c|}{}                                                                               & Clusters(n. user \textgreater 3) & 4 (74.60 \%)                                                                           & 7 (88.2 )\%                                                                         & 11 (89.80 \%)                                                                       & 10 (71.20 \%)                                                                   & 9 (87.90\%)                                                                          & 11 (70.69\%)                                                                       & 10 (86.20\%)                                                                      & 7 (55.20\%)                                                                        \\ \cline{2-10} 
%			\multicolumn{1}{|c|}{}                                                                               & Mean Overlap                     & 38.60 \%                                                                               & 63 \%                                                                               & 48.50 \%                                                                            & 58.60 \%                                                                        & 53.70\%                                                                              & 75 \%                                                                              & 41.10\%                                                                           & 47.20\%                                                                            \\ \cline{2-10} 
%			\multicolumn{1}{|c|}{}                                                                               & Max pop cluster                  & \begin{tabular}[c]{@{}c@{}}1 cl. with 24u.\\ pop. 40.70\%\\ ov. 35.40\%\end{tabular}   & \begin{tabular}[c]{@{}c@{}}1cl with 20u.\\ pop. 33.90\%\\ ov. 59.70\%\end{tabular}  & \begin{tabular}[c]{@{}c@{}}1cl. with 8u\\ pop. 13.80\%\\ ov. 59.20\%\end{tabular}   & \begin{tabular}[c]{@{}c@{}}1cl. with 10u.\\ pop. 17.24\%\\ ov. 0\end{tabular}   & \begin{tabular}[c]{@{}c@{}}1 cl with 9 u\\ pop. 15.50\%\\ ov. 58.60\%\end{tabular}   & \begin{tabular}[c]{@{}c@{}}1 cl. with 7u\\ pop. 17.10\%\\ ov. 72.40\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}2cl with 7u\\ pop. 24.15\%\\ ov. 0\%\end{tabular}      & \begin{tabular}[c]{@{}c@{}}1cl. with 8u.\\ pop. 13.80\%\\ ov. 65.40\%\end{tabular} \\ \hline
			\multicolumn{1}{|c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} {\rotatebox[origin=c]{90}{\small \hspace{0.18cm} Fr. \texttildelow30s}}\end{tabular}}}  & K                                & 10                                                                                     & 15                                                                                  & 10                                                                                  & 15                                                                              & 13                                                                                   & 24                                                                                 & 13                                                                                & 24                                                                                 \\ \cline{2-10} 
		%	\multicolumn{1}{|c|}{}                                                                               & Clusters(n. user \textgreater 3) & 3 (84.75 \%)                                                                           & 5 (76.30 \%)                                                                        & 8 (93.20 \%)                                                                        & 12 (94.90 \%)                                                                   & 9 (89.70\%)                                                                          & 8 (56.90\%)                                                                        & 11 (96.50\%)                                                                      & 7 (50\%)                                                                           \\ \cline{2-10} 
			\multicolumn{1}{|c|}{}                                                                               & Mean Overlap Cl.(\% user \textgreater 3)                   & 38.90 \%    (84.75 \%)                                                                           & \textbf{62.50 \%           (76.30 \%)}                                                                 & 53.95 \%      (93.20 \%)                                                                      & 48.10 \%      (94.90 \%)                                                                  & 46 \%       (89.70\%)                                                                         & \textbf{72.35\%      (56.90\%)}                                                                      & 45.90\%   (96.50 \%)                                                                         & 51.50\%          (50\%)                                                                   \\ \cline{2-10} 
			\multicolumn{1}{|c|}{}                                                                               & 
			Main cl. overlap (\% users)
			& \begin{tabular}[c]{@{}c@{}}%1cl. with 26u.\\ pop. 
				 26.70\% (44.10\%)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}%1cl with 18u\\ pop. 
				\textbf{58.60\% (30.50\%)}\end{tabular}   & \begin{tabular}[c]{@{}c@{}}%1cl with 11u\\ pop. 
				48.30\% (19\% )\end{tabular}      & \begin{tabular}[c]{@{}c@{}}%1cl. with 12u.\\ pop. 
				0\% (20.70\% )\end{tabular} & \begin{tabular}[c]{@{}c@{}}%1 cl with 12u\\ pop. 
				32.90\% (20.70\%) \end{tabular}   & \begin{tabular}[c]{@{}c@{}}%1 with 7u.\\ pop. 
				\textbf{69\% (12.10\% )}\end{tabular}      & \begin{tabular}[c]{@{}c@{}}%1 with 11u\\ pop. 
				15\% (19\% )\end{tabular}         & \begin{tabular}[c]{@{}c@{}}%1 cl. with 8u\\ pop. 
				23.50\% (13.80\%) \end{tabular} \\ \hline 
			\multicolumn{1}{|c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}{\rotatebox[origin=c]{90} {{\hspace{0.3cm}Fr. \texttildelow40s}}}\end{tabular}}} & K                                & 8                                                                                      & 15                                                                                  & 8                                                                                   & 15                                                                              & 18                                                                                   & 27                                                                                 & 18                                                                                & 27                                                                                 \\ \cline{2-10} 
			%\multicolumn{1}{|c|}{}                                                                               & Clusters(n. user \textgreater 3) & 
			%3 (89.83\%)                                                                            & 5 (76.30\%)                                                                         & 
			%8 (100\%)                                                                           & 
			%9 (84.75\%)                                                                     & 
			%7 (75.90\%)                                                                          & 
			%14 (77.60\%)                                                                       & 
			%16 (96.55\%)                                                                      & 18 (84.50\%)                                                                       \\ \cline{2-10} 
			\multicolumn{1}{|c|}{}                                                                               & Mean Overlap Cl.(\% users \textgreater 3)            & 35.60\%  (89.83\%)                                                                                & \textbf{65.75\%   (76.30\%)}                                                                           & 
			44.38\%    (100\%)                                                                          & 
			47.65\%  (84.75\%)                                                                              & 
			47.65 \%  (75.90\%)                                                                           & 
		\textbf{	72.95 \%  (77.60\%)}                                                                         & 60.27\%  (96.55\%)                                                                          & 65.90\%   (84.50\%)                                                                           \\ \cline{2-10} 
			\multicolumn{1}{|c|}{}& Main cl. overlap (\% users)                & 
			\begin{tabular}[c]{@{}c@{}}%1cl. with 27u\\ pop.  \\ ov. 
				24.20\% (45.80\%)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}%1cl. with 21\\ pop. \\ ov.
				\textbf{58.33\% (35.60\%)}\end{tabular}   & \begin{tabular}[c]{@{}c@{}}%1cl. with 18u.\\ pop. \\ ov. 
				0\% (30.50\%)\end{tabular}     & \begin{tabular}[c]{@{}c@{}}%1cl. with 9u.\\ pop. \\ ov. 
				0\% (15.25\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}%1 cl with 12 u.\\ pop. \\ ov. 
				51.80\% (20.70\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}%1 with 10 u.\\ pop. \\ ov. 
			\textbf{	63.70\% (17.24\%)}\end{tabular}  & \begin{tabular}[c]{@{}c@{}}%2 cl with 6u\\ pop. \\ ov.
				47.50\% (20.70\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}%1 cl with 5u.\\ pop. \\ ov.
				33.60\% (8.60\%)\end{tabular}  \\ \hline
			\multicolumn{1}{|c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}{\rotatebox[origin=c]{90} {\hspace{0.3cm}Fr. \texttildelow50s}}\end{tabular}}} & K                                & 8                                                                                      & 12                                                                                  & 8                                                                                   & 12                                                                              & 18                                                                                   & 29                                                                                 & 18                                                                                & 29                                                                                 \\ \cline{2-10} 
			%\multicolumn{1}{|c|}{}                                                                               & Clusters(n. user \textgreater 3) & 
			%3 (89.80\%)                                                                            & 
		%	5 (86.45\%)                                                                         & 
		%	7 (98.30\%)                                                                         & 11 (96.60\%)                                                                    & 7 (77.60\%)                                                                          & 7 (51.70\%)                                                                        & 12 (87.90\%)                                                                      & 9 (55.17\%)                                                                        \\ \cline{2-10} 
			\multicolumn{1}{|c|}{}                                                                               & Mean Overlap Cl.(\% users \textgreater 3)                    & 
			48.20\%  (89.80\%)                                                                              &
			 \textbf{65.70\%   (86.45\%)  }                                                                         & 
			 43.50\%  (98.30\%)                                                                            &
			 55.30\%   (96.60\%)                                                                        & 
			 49.12 \%    (77.60\%)                                                                          & \textbf{71.40\%      (51.70\%)   }                                                                   & 48.36 \%    (87.90\%)                                                                      & 55.90 \%     (55.17\%)                                                                        \\ \cline{2-10} 
			\multicolumn{1}{|c|}{}  &Main cl. overlap (\% users) & 
			\begin{tabular}[c]{@{}c@{}}%1 cl. with 18u.\\ pop.  \\ ov. 
				46.40\%(30.50 \%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}%1cl with 22u.\\ pop.\\ ov
			\textbf{	59.90\% (57.70\%)}\end{tabular}   & \begin{tabular}[c]{@{}c@{}}%1cl with 13u\\ pop. \\ ov.
				0\% (22.40\%) \end{tabular}       & \begin{tabular}[c]{@{}c@{}}%1cl with 9u.\\ pop. \\ ov. 
				0\% (15.25\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}%1 cl with 13u\\ pop. \\ ov. 
				30.60 (22.40\%)\%\end{tabular}   & \begin{tabular}[c]{@{}c@{}}%3 cl with 5 u\\ pop. \\ ov. 
			\textbf{	70.80\% (25.90\%)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}%2 cl with 7 u\\ pop.\\ ov. 
				37\% (24.15\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}%2 cl with 5 u\\ pop. \\ ov. 
				62.71\% (17.24\%)\end{tabular}   \\ \hline
		\end{tabular}%
	}
	\caption{Clustering analysis of users in three selected frames from Rollercoaster (first half) and Timelapse (second half). In brackets, the percentage of covered population. }
	\label{table}
\end{table*}
%\textbf{[Analysis over time toward content analysis]}\\

\begin{figure}[t]
	\centering
	%\subfigure[Rollercoaster video - T = 1 frame]{
	%	\includegraphics[width=0.5\textwidth]{figures/Roller_singleframeclustering.eps}}
	%\subfigure[Timelapse video - T = 1 frame]{
	%	\includegraphics[width=0.5\textwidth]{figures/Time_singleframecl.eps}}
	\subfigure[Rollercoaster video - T = 3 s. ]{
		\includegraphics[width=0.38\textwidth]{figures/Roller_ch90_clRate1_Th60.eps}}
	\subfigure[Timelapse video - T = 3 s.]{
		\includegraphics[width=0.38\textwidth]{figures/Time_ch90_clRate1_Th60.eps}}
	\caption{\label{fig:AllVideo_OvInter_Var} Mean and variance of the joint overlap across clusters over time. In the legend, the mean value of joint viewport overlap of clusters with more than three users performed across the entire video.}
\end{figure}
{\textbf{Trajectory-based clustering.} } Second, we test the proposed algorithm over a time-window of duration $T = 3s$ and similarity threshold $\tau = 1.8s $. %(i.e., users are set as neighbors if they are it for at least the 60\% of the time-window). 
 In this case, we compare the proposed solution with SC algorithm~\cite{Gwendal2018}. %The clustering is  performed with trajectories lasting the  entire video. To make a fair comparison,
 The latter is applied in the following conditions: $i)$ to trajectories spanning the entire video as in~\cite{Gwendal2018}, $ii)$ consecutive time windows of duration $T$ and $iii)$ imposing the same $K$ obtained from our solution (``SC - K given"). Fig.~\ref{fig:AllVideo_OvInter_Var} shows results in terms of overlap % the mean and variance of the overlap 
 among viewports clustered together in both Rollercoster (a) and Timelapse (b).
In more details, all users are clustered over consecutive time-windows of $T$ seconds each. %optimal clusters are evaluated.
 Then, for each frame the viewport overlap among all users within one cluster is evaluated and averaged across clusters. The mean overlap (solid line) and the variance (shaded area) is finally depicted in Fig.~\ref{fig:AllVideo_OvInter_Var}.  Moreover, the mean value of joint overlap in clusters with more than three users across the entire video is shown in the legend. Our solution outperforms SC in terms of mean overlap but also in terms of variance. The latter shows the stability of our clustering method ensuring for each cluster a consistent overlap over time. Finally, the performance gain is significant also in terms of overlap in the most populated clusters (value provided in the legend). 
 
	

